Hiring Secretaries over Time: The Benefit of Concurrent Employment

We consider a stochastic online problem where $n$ applicants arrive over time, one per time step. Upon arrival of each applicant their cost per time step is revealed, and we have to fix the duration of employment, starting immediately. This decision is irrevocable, i.e., we can neither extend a contract nor dismiss a candidate once hired. In every time step, at least one candidate needs to be under contract, and our goal is to minimize the total hiring cost, which is the sum of the applicants' costs multiplied with their respective employment durations. We provide a competitive online algorithm for the case that the applicants' costs are drawn independently from a known distribution. Specifically, the algorithm achieves a competitive ratio of 2.965 for the case of uniform distributions. For this case, we give an analytical lower bound of 2 and a computational lower bound of 2.148. We then adapt our algorithm to stay competitive even in settings with one or more of the following restrictions: (i) at most two applicants can be hired concurrently; (ii) the distribution of the applicants' costs is unknown; (iii) the total number $n$ of time steps is unknown. On the other hand, we show that concurrent employment is a necessary feature of competitive algorithms by proving that no algorithm has a competitive ratio better than $\Omega(\sqrt{n} / \log n)$ if concurrent employment is forbidden.

==> 11_related.tex <==

\paragraph{Further related Work}
\label{sec:related}

However, most of them are maximization problems, where one aims at selecting items in order to maximize a certain objective function.

In our work, we consider minimization problems. They provide quite a different structure, as beside to the goal of minimizing the objective function one has to keep given covering constraints in every time step. Beside the Ski Rental problem, introduced in~\cite{karlin1986} and investigated in variantsin, e.g., \cite{khanafer2013,lotker2008,lotker2012rent}, there are two more well-known online minimization problems: the Parking Permit~\cite{meyerson2005} Problem, which generalizes Ski Rental, and the Facility Leasing Problem~\cite{anthony07,nagarajan2013}. As stated in~\cite{kniesburges2014}, the Parking Permit Problem serves as a basis for all other currently considered online leasing problems. Further, algorithms designed to solve online leasing problems are consistently built upon algorithms for the corresponding non-leasing variants of the respective problems~\cite{kniesburges2014}.

Both is not the case with the Secretary Leasing, as it differs in its structure and goals from Parking Permit as well as from Facility Leasing. In the Secretary Leasing problem, we know the length $n$ of the input, but the incoming cost are stochastic. Furthermore, we are not forced to choose our strategy from a given set, but we are allowed to freely decide for how long we want to employ a secretary. This corresponds to a strategy space of size $n$ in the Parking Permit Problem, where the number of possible actions is usually bounded by some constant $k$. In the Facility Leasing problem, the cost structure is different: in addition to the leasing cost a connection cost is charged, and this latter one is not always the same for a fixed incoming item, but depends on where the nearest opened facility is. And again, the strategy space in Secretary Leasing is larger as we do not choose the leasing durations from a given set.

Although all of the above mentioned problems have the use of stochastic arrival in common, there are differences in how these models are exactly defined. Where \cite{kleinberg2005,babaioff07,kesselheim2013}, e.g., assume the input to be constructed adversarially and then be presented in random order, \cite{kleinberg2012,alaei2012} allow adversarial construction and presentation, but make use of probability distributions to determine the exact outcome (e.g. a node weight) upon arrival. In~\cite{goebel2014} a model is introduced that allows to cover multiple stochastic arrival models and, thus, shows them to be similar regarding their power. In this work, we only use probability distributions and do not have any fixed adversarial components. The distributions, however, are allowed to be arbitrary and the algorithm does not need much knowledge about them. \todo{spezifizieren, was genau bekannt sein muss.}
\todo{noch mehr related work zu online algorithms mit prob. distributions?}

%%%%%%%%%% andere Quellen die nur mit Verteilungen arbeiten ??
%%%%%%%%%% Abgrenzung der Mächtigkeiten; können Verteilungen weniger als random permutations? Ist das hier interessant?


%\paragraph{Related Work}
%\label{sec:related}
%
%The history of the original Secretary Problem dates back until at least the 1960s, when Dynkin~\cite{dynkin} and Lindley~\cite{lindley} gave an optimal $\nicefrac{1}{e}$-competitive algorithm for the problem of selecting the maximum value online from a random sequence of numbers. 
%The Secretary Problem does not allow for good bounds in terms of competitive analysis.
%The problem is usually studied with respect to stochastic arrival models.
%%This is an example where the classical online worst-case analysis, as it is often conducted in the field of paging or list accessing problems, immediately fails. It is easy to construct lower bounds of $\Omega(n)$ for the Secretary Problem and related questions.
%Problems based on the Secretary Problem \cite{kleinberg2005} \todo{noch mehr secr. paper zitieren?} as well as non-trivial optimization problems were considered, see, e.g.,  \cite{babaioff07,kesselheim2013,babaioff2007soda,kleinberg2012,alaei2012,meyerson2001}. However, most of them are maximization problems, where one aims at selecting items in order to maximize a certain objective function.
%
%In our work, we consider minimization problems. They provide quite a different structure, as beside to the goal of minimizing the objective function one has to keep given covering constraints in every time step. Beside the Ski Rental problem, introduced in~\cite{karlin1986} and investigated in variantsin, e.g., \cite{khanafer2013,lotker2008,lotker2012rent}, there are two more well-known online minimization problems: the Parking Permit~\cite{meyerson2005} Problem, which generalizes Ski Rental, and the Facility Leasing Problem~\cite{anthony07,nagarajan2013}. As stated in~\cite{kniesburges2014}, the Parking Permit Problem serves as a basis for all other currently considered online leasing problems. Further, algorithms designed to solve online leasing problems are consistently built upon algorithms for the corresponding non-leasing variants of the respective problems~\cite{kniesburges2014}.
%
%Both is not the case with the Secretary Leasing, as it differs in its structure and goals from Parking Permit as well as from Facility Leasing. In the Secretary Leasing problem, we know the length $n$ of the input, but the incoming cost are stochastic. Furthermore, we are not forced to choose our strategy from a given set, but we are allowed to freely decide for how long we want to employ a secretary. This corresponds to a strategy space of size $n$ in the Parking Permit Problem, where the number of possible actions is usually bounded by some constant $k$. In the Facility Leasing problem, the cost structure is different: in addition to the leasing cost a connection cost is charged, and this latter one is not always the same for a fixed incoming item, but depends on where the nearest opened facility is. And again, the strategy space in Secretary Leasing is larger as we do not choose the leasing durations from a given set.
%
%Although all of the above mentioned problems have the use of stochastic arrival in common, there are differences in how these models are exactly defined. Where \cite{kleinberg2005,babaioff07,kesselheim2013}, e.g., assume the input to be constructed adversarially and then be presented in random order, \cite{kleinberg2012,alaei2012} allow adversarial construction and presentation, but make use of probability distributions to determine the exact outcome (e.g. a node weight) upon arrival. In~\cite{goebel2014} a model is introduced that allows to cover multiple stochastic arrival models and, thus, shows them to be similar regarding their power. In this work, we only use probability distributions and do not have any fixed adversarial components. The distributions, however, are allowed to be arbitrary and the algorithm does not need much knowledge about them. \todo{spezifizieren, was genau bekannt sein muss.}
%\todo{noch mehr related work zu online algorithms mit prob. distributions?}

%%%%%%%%%% andere Quellen die nur mit Verteilungen arbeiten ??
%%%%%%%%%% Abgrenzung der Mächtigkeiten; können Verteilungen weniger als random permutations? Ist das hier interessant?

























